DeepTest Tool Competition 2026: Benchmarking an LLM-Based Automotive Assistant

This report summarizes the results of the first edition of the Large Language Model (LLM) Testing competition, held as part of the DeepTest workshop at ICSE 2026. Four tools competed in benchmarking an LLM-based car manual information retrieval application, with the objective of identifying user inputs for which the system fails to appropriately mention warnings contained in the manual. The testing solutions were evaluated based on their effectiveness in exposing failures and the diversity of the discovered failure-revealing tests. We report on the experimental methodology, the competitors, and the results.

==> TODO.tex <==
ranking
- experiments: 6 x 2h = 12h -> one approach
- two manuals -> 24h
- run in parallel approaches? RAG latency?
-> in one day doable?

judge
- rerun judges 6 times on Samueles dataset

decide config:
- oracle: gpt-4o?
- generator: gpt-4o-mini
- sut: gpt-5-chat?

final setup:
- 4 tools
- 2 llms (GPT-4o-mini, DeepSeek)
- 2 suts (industrial, competition)
- 2 manuals (MINI, BMW)
- 2 languages (AE, BE): Optional
- 6 times

---------------
96 hours - 4 days (two llms)
48 hours - 2 day (1 llm)
----------------
or parallelize seeds with other pc
-------------
Tuesday - gpt-4o-mini. real
Wed - gpt-4o-mini. dummy

Wed - gpt-4o-mini. mini real
Thursday - gpt-4o-mini. mini. dummy

Thursday - DeepSeek-V3. real
Friday - DeepSeek-V3. dummy

Friday - DeepSeek-V3. mini. real
Saturday - DeepSeek-V3. mini. dummy

Sunday - Coverage, Paper
Monday - Paper

---------------------------------
Code
-------------------
coverage
boxplots effectiveness

------
dummy
--------
gpt-4o-mini
deepseek-v3
gpt-5-chat
------
carexpert
------
gpt-4o-mini
gpt-5
-----------

final
----------------
- include coverage scores
- include GPT-5-Chat results
- remove failure count from S/Text
- update plots
- formatting
- shorten
- related work
- statistical tests?

